Affinely Connected Spaces, Geodesic Loops, $G_2$-Structures and Deformations

We investigate octonion product deformations coming from the parallelizable torsion of the 7-sphere $S^7$, obtaining a family of geometries from solutions of the Lagrangian formalism movement equations. This can be achieved by analyzing the spontaneous compactification $M_4\times S^7$, where $M_4$ is a Lorentzian $4$-dimensional manifold. Besides the usual Riemannian geometry and two others proposed by Cartan and Schouten, solutions in geometries with torsion and more general seven-dimensional spaces are obtained. Such formalism may by subsequently derived over the 7-sphere $S^7$, locally given by the structure constants of a nonassociative geodesic loop. Furthermore, $G_2$-structures are investigated, giving rise to the octonion product and bundle $\mathbb{O} M$ over a seven-dimensional manifold $M$. Then, sections of this bundle over such space can be perceived as spinor fields in an isometric identification mapping the spin connection to an octonion covariant derivative preserving the octonion product defined over $\mathbb{O} M$.

==> folha-de-aprovacao.tex <==
% Este arquivo não deve ser utilizado.
\begin{center}
  {\Large \textbf{FOLHA DE APROVAÇÃO}
  }
\end{center}





Escaneie a folha de aprovação e
sobre-escreva o arquivo \verb+folha-de-aprovacao.pdf+.

